WonderJourney: Going from Anywhere to Everywhere

We introduce WonderJourney, a modularized framework for perpetual 3D scene generation. Unlike prior work on view generation that focuses on a single type of scenes, we start at any user-provided location (by a text description or an image) and generate a journey through a long sequence of diverse yet coherently connected 3D scenes. We leverage an LLM to generate textual descriptions of the scenes in this journey, a text-driven point cloud generation pipeline to make a compelling and coherent sequence of 3D scenes, and a large VLM to verify the generated scenes. We show compelling, diverse visual results across various scene types and styles, forming imaginary "wonderjourneys". Project website: https://kovenyu.com/WonderJourney/

==> fig_tex/ablation_text.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ablation_text.pdf}
    \vspace{-0.6cm}
    \caption{\footnotesize\textbf{Ablation on text prompts by LLM.} 
    Without the LLM to generate scene text, the journey always stays in a village. LLM increases scene diversity (e.g., snowfield, river).
    }
    \label{fig:ablation_text}
    \vspace{-0.3cm}
\end{figure}

==> fig_tex/full_3d.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/full_3d.pdf}
    \vspace{-0.7cm}
    \caption{\footnotesize\textbf{Full 3D consistency.} The tower re-appears since we maintain full 3D consistency with a single point cloud.}
    \label{fig:full_3d}
    \vspace{-0.6cm}
\end{figure}

==> supp_text/reproducibility_statement.tex <==
\section{Reproducibility Statement}\label{sec:reproduce}
To facilitate future research, we will release code upon acceptance. Note that our framework is fully modular, and the components, such as LLM, VLM, depth estimator, and outpainter, can be readily replaced by more advanced models in the future.

==> text/1_intro_short.tex <==
\vspace{-10pt}
\begin{flushright}
``No, no! The adventures first, explanations take such a dreadful time.'' -- \emph{Alice's Adventures in Wonderland}
\end{flushright}


\section{Introduction}
\aftersec

In %
``Alice's Adventures in Wonderland'', the story begins with Alice falling down the rabbit hole and emerging into a strange and captivating Wonderland. In her journey through this wonderland, Alice encounters many 
curious characters
such as the Cheshire Cat and the Mad Hatter,
and peculiar scenarios, such as the tea party and the rose garden -- eventually ending at the royal palace. These characters and settings combine to form a compelling world that has fascinated countless readers over the years. In this paper, we follow in this creative tradition and explore how modern computer vision and AI models can similarly generate such interesting and varied visual worlds, which users can journey through, much like Alice did in her own adventures in Wonderland. 

Toward this goal, we introduce the problem of \emph{\problem}. Unlike previous work on perpetual view generation~\citep{liu2021infinite,li2022infinitenature} that only generates a single type of scene, such as nature photos, our objective is to synthesize a series of diverse 3D scenes starting at an arbitrary location specified via a single image or language description. The generated 3D scenes should be \emph{coherently connected} along a long-range camera trajectory, traveling through various plausible places. The generated 3D scenes allow rendering a fly-through video through a long series of diverse scenes to simulate the visual experience of a journey in an imaginary ``wonderland''. We show examples in \fig{\ref{fig:teaser}}. 

The main challenges of \problem center around generating \emph{diverse yet plausible} scene elements. These scene elements need to support the formation of a path through coherently connected 3D scenes. They should include various objects, backgrounds, and layouts that fit in observed scenes and transit naturally to the next, yet unobserved, scenes. This generation process can be broken down into determining what objects to generate for a given scene; where to generate these objects; and how these scenes connect to each other geometrically. Determining what elements to generate calls for semantic understanding of a scene (e.g., a lion might not be a great fit for a kitchen); determining where to generate them calls for common sense regarding the visual world (e.g., a lion should not be floating in the sky); further, generating these elements in a new connected scene requires geometric understanding (e.g., occlusion and disocclusion, parallax, and appropriate spatial layouts). Notably, these challenges are absent in prior work on perpetual view generation, as they tend to focus on a single domain~\citep{liu2021infinite} or a single scene~\citep{fridman2023scenescape}.

Our proposed solution, \modelfull, addresses each of the above challenges in \problem with its own module. \model leverages an LLM to generate a long series of scene descriptions, followed by a text-driven visual scene generation module to produce a series of colored point clouds to represent the connected 3D scenes. 
Here, the LLM provides commonsense and semantic reasoning; the vision module provides visual and geometric understanding and the appropriate 3D effects. In addition, we leverage a vision-language model (VLM) to verify the generation and launch a re-generation when it detects undesired visual effects. Our framework is fully modularized. Each of the modules can be implemented by the best pretrained models, allowing us to leverage the latest and future advancements in the rapidly growing vision and language research.
Our main contributions are as follows:
\vspace{0.1cm}
\begin{itemize}
    \item We study \problem and propose \model, a fully modularized framework that decomposes this problem into core components: an LLM to generate scene descriptions, a text-driven visual module to generate the coherent 3D scenes, and a VLM to verify the generated scenes.
    \vspace{0.05cm}
    \item We design a visual scene generation module that leverages off-the-shelf text-to-image and depth estimation models to generate coherent 3D point clouds. Our module handles boundary depth inaccuracy, sky depth inaccuracy, and dis-occlusion unawareness.
    \vspace{0.05cm}
    \item We show compelling visual results and compare \model with SceneScape~\citep{fridman2023scenescape} and InfiniteNature-Zero~\citep{li2022infinitenature} in a user study, which shows that \model produces interesting and varied journeys. %
    
\end{itemize}


==> text/2_rw_short.tex <==


\input{fig_tex/overview}
\section{Related Work}
\aftersec

\myparagraph{Perpetual view generation.}
The seminal work on perpetual view generation is Infinite Images \cite{kaneva2010infinite} which synthesizes the effect of navigating a 3D world by stitching and rendering images according to camera motions.
Later works, such as Infinite Nature~\cite{liu2021infinite} and InfiniteNature-Zero~\cite{li2022infinitenature}, learn to auto-regressively generate next view based on the current view. 
Follow-up works improve global 3D consistency~\citep{chai2023persistent} and visual quality~\cite{cai2022diffdreamer}. %
A recent work, SceneScape~\cite{fridman2023scenescape}, explores text-driven perpetual view generation by gradually constructing a single cave-like scene represented by a lengthy mesh.
While these methods study perpetual generation, they are restricted to a single domain such as nature photos~\cite{liu2021infinite,li2022infinitenature} or a single scene~\cite{fridman2023scenescape}.



\myparagraph{3D scene generation.}
Considerable progress has recently been made in text-to-3D or image-to-3D generation, many of which focus on objects without background~\cite{poole2022dreamfusion, raj2023dreambooth3d,liu2023zero,melas2023realfusion, lin2023magic3d, li20223ddesigner, cheng2023sdfusion}. 
These works typically leverage a 2D image prior from an image generation model, e.g., an image diffusion model~\cite{rombach2022high}, and then build a 3D representation, such as a NeRF~\cite{wang2021nerf}, by distilling the supervision of the 2D image generation model~\citep{poole2022dreamfusion}.
Other works on 3D object generation focus on learning a 3D generative model directly from 2D images~\citep{chan2022efficient, chan2021pi, gu2021stylenerf, hao2021gancraft, nguyen2019hologan, niemeyer2021giraffe, or2022stylesdf, schwarz2022voxgraf, sargent2023vq3d}. 

Several works also focus on generating a single 3D scene with background~\cite{devries2021unconstrained,bautista2022gaudi}. 
For example,
Text2Room~\cite{hollein2023text2room} generates a room-scale 3D scene from a single text prompt, using textured 3D meshes for their scene representation.
Other relevant works have focused on generating (sometimes called ``reconstructing'') a scene from limited observations, such as a single image. Long-Term Photometric Consistent NVS~\cite{yu2023long} generates single scenes from a source image by auto-regressively generating with a conditional diffusion model. 
GeNVS~\cite{chan2023genvs} and Diffusion with Forward Models~\cite{tewari2023diffusion} use an intermediate 3D representation but are trained and evaluated on each scene separately. ZeroNVS~\cite{sargent2023zeronvs} synthesizes a NeRF of a scene from a single image.
Their work focuses on generating a single scene while ours targets generating a coherently connected sequence of diverse scenes.

\myparagraph{Text-guided video generation.}
The idea of scene generation has also been explored in video generation. Several concurrent works like TaleCrafter~\cite{gong2023talecrafter} and others~\cite{liu2023intelligent,huang2023free,lin2023videodirectorgpt} also discuss the task of creating a series of videos which follow an LLM-generated story or script. However, all these works use different scenes as different clips in a video, resulting in hard cuts, while our \problem aims at generating sequences of coherently connected scenes.

\ignore{
\myparagraph{Depth and Segmentation Estimation.}
Though our paper is about \problem, we make extensive use of the estimation literature


- Need to put some of the papers that we use here e.g. MIDAS, Zoe-Depth, SAM, and discuss that despite the progress there are still failures.
}

==> text/3_method_short.tex <==

\input{fig_tex/vision_part}
\section{Approach}
\aftersec


Our goal is to generate a potentially endless sequence of diverse yet coherently connected 3D scenes, which requires both geometric understanding of 3D scenes and visual common sense and semantic understanding of scene structures.
To tackle this challenging task, we propose \modelfull. The main idea is to generate a text description of the visual elements the next scene would contain, and then employ a text-guided visual generation module to make that 3D scene. 

\model is a fully modularized framework that decomposes this task into \llmpart, \visionpart, and \vlmpart, as in \fig{\ref{fig:overview}}. Given an input image or text, we first pair it with the other modality by generating the image with a text-to-image model or by generating the description with a Vision Language Model (VLM). Then we generate the next-scene description by a Large Language Model (LLM). A visual scene generation module takes in the next-scene description and the current scene image to generate the next 3D scene represented by a colored point cloud. This generation process is then checked by a VLM to make sure there is no unwanted effects, or it gets regenerated. We note that our framework is highly modularized, such that each module can be implemented with the latest (pretrained) models and thus can easily leverage the quick advances of large language and vision models. 










\subsection{Scene description generation}
\aftersubsec






We propose an auto-regressive scene description generation process, i.e., the \llmpart~ takes a set of past and current scene descriptions as input and predicts the subsequent scene description:
\aroundeqn
\begin{align}
    \mathcal{S}_{i+1} & = g_\text{description}(\mathcal{J}, \mathcal{M}_i),
\end{align}
\aroundeqn
where $\mathcal{S}_{i}$ denotes the $i^\text{th}$ scene description, and $g_\text{description}$ denotes the scene description generator which is implemented by an LLM that takes two inputs: 
1) the task specification $\mathcal{J}$ = \textit{``You are an intelligent scene generator. Please generate 3 most common entities in the next scene, along with a brief background description.''}; and 2) the scene description memory $\mathcal{M}_{i} = \{\mathcal{S}_0, \mathcal{S}_1, \cdots, \mathcal{S}_i\}$ which is a collection of past and current scenes. The latest description memory is:
\aroundeqn
\begin{align}
    \mathcal{M}_{i+1} & = \mathcal{M}_i \cup \{\mathcal{S}_{i+1}\}.
    \label{eqn:memory}
\end{align}
\aroundeqn
We define the scene description $\mathcal{S}_i \!=\! \{ S, O_i, B_i \}$, which consists of a style $S$ that is kept consistent across scenes, objects in the scene $O_i$, and a concise caption $B_i$ describing the background of the scene. We allow the LLM to output natural language descriptions, and then use a lexical category filter to process the raw text of $O_i$ and $B_i$ such that we only keep nouns for entities and adjectives for attributes. Empirically this generates more coherently connected scenes compared to requiring the LLM to directly output this structured description.

\ignore{
\ky{Decide if we really want this empirical note to appear here. It seems to be a bit distracting to me. I prefer leaving this to supplement as a fun fact in 2023.} In our explorations, we empirically find potential disruptions induced by the inclusion of uncommon objects within textual descriptions, a factor that can detrimentally impact the 3D spatial quality quality of the generated scenes. For instance, an uncommon object "phone booth" has a high likelihood of being generated, leading to its placement in undesired and nonsensical locations, such as the middle of a road or floating in the sky. To address this, we propose instructing the LLM to prioritize providing "most common" objects, as mentioned in $\mathcal{J}$. 
}

\subsection{Visual scene generation}
\aftersubsec
Since we want the generated next scene to be coherent with past scenes geometrically and semantically, we formulate our \visionpart~ as a conditional generation problem, taking both the next-scene description and the 3D representation of the current scene as conditions: 
\aroundeqn
\begin{align}
    \mathcal{P}_{i+1} = g_\text{visual}(I_i, \mathcal{S}_{i+1}),
\label{eqn:visual}
\end{align}
\aroundeqn
where $\mathcal{P}_{i}$ denotes a colored point cloud that represents the next 3D scene, and $I_i$ denotes the image of current scene. The visual scene generator $g_\text{visual}$ consists of learning-free operations such as perspective unprojection and rendering, as well as components that use parametric (pretrained) vision models, including a depth estimator, a segmentation-based depth refiner, and a text-conditioned image inpainter. We show an illustration in \fig{\ref{fig:vision_part}}.

\myparagraph{Lifting image to point cloud.}\label{sec:imagetopointcloud}
Given the current scene represented by an image $I_i$, we lift it to 3D by estimating depth and unproject it with a pinhole camera model. We use MIDAS v3.1 \cite{Ranftl2022}, one of the state-of-the-art depth estimators, in our experiments. However, we find that existing monocular depth estimators share two common issues. First, depth discontinuity is not well modeled, witnessed by previous work~\citep{tosi2021smd,aleotti2021neural,miangoleh2021boosting}, resulting in overly smooth depth edges across object boundaries. Second, the depth of the sky is always underestimated, also observed by previous work~\citep{liu2021infinite,li2022infinitenature}. To address these two issues, we introduce a depth refinement process that leverages pixel grouping segments and sky segmentation.


\input{fig_tex/diverse_results}

\myparagraph{Depth refinement.} To enhance the depth discontinuity across object boundaries, we model scene elements with frontal planes when the elements have a limited disparity range. We use SAM~\citep{Kirillov_2023_ICCV} to generate pixel grouping segments $\{\texttt{seg}_j\}_{j=1}^{N_s}$ where $\texttt{seg}_j\in\{0,1\}^{H\times W}$ is a segment mask, sorted in descending order according to the size of the segment $\lVert \texttt{seg}_j \rVert$. We iteratively refine the estimated depth:
\begin{align}
\small
    \!\!\!\!\! \texttt{depth}[\texttt{seg}_j] \! \leftarrow  \!
    \begin{cases} 
\texttt{median}(\texttt{depth}[\texttt{seg}_j]), & \text{if } \Delta D_j \!<\! T, \\
\texttt{depth}[\texttt{seg}_j], & \text{otherwise},
    \end{cases}
\end{align}
for $j=1,\cdots, N_s$, where $\texttt{depth}\in \R_{+}^{H\times W}$ is initialized with the estimated monocular depth, $\texttt{median}(\cdot)$ is a function that returns the median value of the input set, $\Delta D_j=\texttt{max}(\texttt{disparity}[\texttt{seg}_j]) - \texttt{min}(\texttt{disparity}[\texttt{seg}_j])$ denotes the disparity (the reciprocal of \texttt{depth}) range within the segment $\texttt{seg}_j$. We keep the estimated depth of segments with high disparity range as they do not fit to a frontal-plane, such as roads. Note that the idea of frontal-plane modeling has also been explored in 3D Ken-Burns~\citep{niklaus20193d} with selected semantic classes such as car and people. 
In contrast, as we target at general scenes with diverse styles, we use the criterion of the disparity range for keeping estimated depth instead of selected semantic classes.

To handle the sky depth which is always underestimated, we use OneFormer~\citep{jain2023oneformer} to segment sky region and assign a high depth value to it. However, this results in inaccurate depth estimates along the sky boundary; if we were to naively use the output segmentation, these errors result in accumulated severe artifacts in later scenes. To resolve it, we simply remove points along the sky boundary. Besides, we find that depth at distant pixels are generally not reliable. Thus, we also set a far background plane with depth $F$ that cuts off all pixels' depth beyond it.

\myparagraph{Description-guided scene generation.}\label{sec:vision}
To generate a new scene that is connected to the current scene, we place a camera $C_{i+1}$ with an appropriate distance to the current camera $C_i$. 
As shown in \fig{\ref{fig:vision_part}}, we render the partial image $\hat{I}_{i+1}$ and inpaint it with a text-guided inpainter to generate a new scene image $I_{i+1}$:
\aroundeqn
\begin{align}
    I_{i+1} = g_\text{inpaint}(\hat{I}_{i+1}, \mathcal{S}_{i+1}),
\end{align}
\aroundeqn
where we use the Stable Diffusion inpainting model~\citep{rombach2022high} for $g_\text{inpaint}$ in our experiments. 
Note, we purposefully place the new camera at a location that creates enough empty space in the rendered image. We empirically find that text-guided inpainters tend to avoid generating partial objects, likely due to their curated training image datasets, which tend to not include truncated or partial objects. Leaving too little empty space therefore results in just a simple extrapolation of the partial image $\hat{I}_{i+1}$ and a lack of adherence to the text prompt $\mathcal{S}_{i+1}$, especially in regards to new objects. After generating the new scene image, we lift it to 3D by estimating and refining depth for it, and we obtain the new point cloud $\hat{\mathcal{P}}_{i+1} = \mathcal{P}_i \cup \mathcal{P}'_{i+1}$ where $\mathcal{P}'_{i+1}$ denotes the additional points from unprojecting the inpainted pixels.


\myparagraph{New scene registration by depth consistency.} However, as the depth estimator is unaware of geometry constraints, the depth for points in $\mathcal{P}'$ generally do not align with $\mathcal{P}_i$. Thus, we adapt the depth estimator by a depth alignment loss:
\aroundeqn
\begin{align}
\footnotesize
    \Loss_\text{depth} = \max(0, \mathcal{D}^*_\text{bg}-\mathcal{D}'_\text{bg}) + \lVert\mathcal{D}^*_\text{fg}-\mathcal{D}'_\text{fg}\rVert,
\end{align}
\aroundeqn
where $\mathcal{D}^*_\text{bg}$ denotes the analytically computed depth of background pixels from $I_i$, $\mathcal{D}'_\text{bg}$ denotes the estimated depth for pixels corresponding to $\mathcal{D}^*_\text{bg}$, $\mathcal{D}^*_\text{fg}$ denotes the computed depth of all other visible pixels from $I_i$, and $\mathcal{D}'_\text{fg}$ denotes the estimated depth for pixels corresponding to $\mathcal{D}^*_\text{fg}$.

\myparagraph{Occlusion handling by re-rendering consistency.}
Another geometric inconsistency is that disocclusion regions can have a lower depth values than their occluders, as the depth estimator is not aware of this 3D geometric constraint. We highlight the wrongly estimated disocclusion depth in the refined depth in \fig{\ref{fig:vision_part}}. To resolve this issue, we re-render the new scene $\hat{\mathcal{P}}_{i+1}$ at the camera $C_i$ and detect all inconsistent pixels. At each inconsistent pixel, we move back all the rasterized additional points from $\mathcal{P}'_{i+1}$ that have lower depth values than the one point from $\mathcal{P}_i$. This removes the disocclusion inconsistency and guarantees that the disocclusion comes after the occluder.

\myparagraph{Scene completion.}
We obtain the final point cloud $\mathcal{P}_{i+1}$ by adding more points to $\hat{\mathcal{P}}_{i+1}$. We add points by repeating the following ``complete-as-you-go'' process: we place an additional camera along a camera trajectory connecting the new scene to the current scene, render a partial image at that camera, inpaint the image, and add the additional points to the point cloud.
Note that in our visual scene generation formulation in \eqn{\ref{eqn:visual}}, one can replace the image input $I_i$ with the point cloud $\mathcal{P}_i$ from the current scene, forming a persistent scene representation. This allows a trade-off between 3D persistence and empirical requirements. In practice, maintaining a large point cloud leads to prohibitively many points that require a large amount of GPU memory when generating a long trajectory of high-resolution scenes. Thus in our experiments we take the image formulation.

\input{fig_tex/main_results_v2}

\subsection{Visual validation}
\aftersubsec



\ignore{Occasionally, we encounter undesirable geometry in the generated scene images, such as photo borders, frames, or out-of-focus blurry objects. Thus, we propose a validation step to identify and reject these undesired generated scenes.}

Empirically, in a large portion of generated photos and paintings, a painting frame or a photo border appears, disrupting the geometry consistency. Additionally, there are often unwanted blurry out-of-focus objects near the borders of the generated images. Thus, we propose a validation step to identify and reject these undesired generated scenes.

We formulate this as a text-based detection problem, where our objective is to detect a set of predefined undesirable effects in the generated scene image. We reject and regenerate the scene image if any unwanted effect is detected. Specifically, right after we generate a new scene image $I_{i+1}$, we immediately feed it to a VLM and prompt it with the query $\mathcal{J}^t_\text{detect}$ = \textit{``Is there any $X_t$ in this image?''} where $X_t\in \{ X_1, \cdots, X_T\}$ is an unwanted effect specified by text, such as ``photo border'', ``painting frame'', or ``out-of-focus objects''. If any unwanted effect is detected, we regenerate $I_{i+1}$ with a new description $\mathcal{S}_{i+1}$ or a new random seed. 


\ignore{ \ky{we cannot address this; maybe leave it as a limitation.}
\myparagraph{Floaters from incomplete objects}
- Talk about how there are a few objects that can be generated incompletely. Namely trees. These objects need to be identified and removed, otherwise the depth warping can cause them to ``float'' in the next key-frame. }


==> text/4_exp_short.tex <==
\input{fig_tex/baseline}
\section{Experiments}
\aftersec



\myparagraph{Dataset and baselines.}
Since the \problem is a new task without an existing dataset, we use a mixture of photos taken by ourselves, copyright-free photos from online, and generated examples, for evaluation in our experiments. We perform the pairing process by DALL-E 3~\citep{betker2023improving} for text-to-image pairing. 
We consider two state-of-the-art perpetual view generation methods as our baseline: image-based InfiniteNature-Zero and text-based SceneScape. %


\myparagraph{Qualitative demonstration.}
We show qualitative examples of the generated journey across different scenes and different styles in \fig{\ref{fig:teaser}} and \fig{\ref{fig:main_results}}. These results show that \model is able to generate diverse yet coherently connected scenes from various types of input images, i.e., it can go from anywhere. We show more examples in the Appendix. We further show examples of diverse generation samples from the same input in \fig{\ref{fig:diverse_results}}. These diverse generated journeys suggest that \model supports going to different destinations at each run.

\input{tbl_tex/human_preference}

\myparagraph{Human preference evaluation.}
Since a main application of \model is for creative and entertainment purposes, we focus on human preference evaluation as our quantitative metrics, using the following four axes: diversity of generated scenes in a single journey, visual quality, scene complexity, and overall interesting-ness.
We generate videos following each approach's own camera trajectories setup. 
Since InfiniteNature-Zero is trained on nature photos, we only compare to it using photorealistic nature images. We use $3$ examples for comparison with InfiniteNature-Zero. For SceneScape, since it is text-based, we can use $3$ examples of different styles for comparison. 
We show a side-by-side comparison of videos generated by \model and a baseline with randomized positions. We then ask one binary-choice question at a time, such as \textit{``Compare the two videos below. Which video has a higher \textbf{diversity}? That is, which video shows more various different places?''}.
We recruited $400$ participants, $200$ for the comparison with InfiniteNature-Zero and $200$ for SceneScape. Each participant answers $12$ questions. 

As shown in \tbl{\ref{tbl:human}}, \model is strongly preferred over both baselines on all four axes. 
InfiniteNature-Zero synthesizes only nature scenes, as shown in \fig{\ref{fig:baseline}}, while \model generates more diverse scenes and objects such as mountaineers and houses that are naturally connected to the starting nature scene. SceneScape tends to generate cave-like scenes due to the usage of a textured mesh, and thus all examples converges to caves. Also, as discussed in Section~\ref{sec:vision}, SceneScape tends to not generate new objects due to limited white space. All these factors might contribute to the much greater user preference for \model.







\myparagraph{Limitations.} The rendered videos may have artifacts due to estimation errors (depth, segmentation, etc.), as discussed in Section~\ref{sec:imagetopointcloud}. %
We refine the depth using segmentation, which may also contain errors that result in artifacts. As these networks improve, our techniques should improve too due to our modular design.


==> text/5_conclusion_short.tex <==
\section{Conclusion}
\aftersec
\vspace{0.2cm}

We introduce \modelfull to generate a long sequence of diverse yet coherently connected 3D scenes starting at any user provided location.
\modelfull achieves compelling, diverse visual results across various scene types and different styles, enabling users to journey through their own adventures in the generated ``wonderjourneys''.


